Addressing Mixed Traffic Through Platooning of Vehicles

Connected and automated vehicles (CAVs) provide the most intriguing opportunity for enabling users to better monitor transportation network conditions and make better operating decisions to improve safety and reduce pollution, energy consumption, and travel delays. While several studies have shown the benefits of CAVs in reducing energy and alleviating traffic congestion in specific traffic scenarios, e.g., crossing signal-free intersections, merging at roadways and roundabouts, cruising in congested traffic, passing through speed reduction zones, and lane-merging or passing maneuvers, most of these efforts have focused on 100% CAV penetration rates without considering human-driven vehicles (HDVs). One key question that still remains unanswered is ``how can CAVs and HDVs be coordinated safely?'' In this paper, we report on an optimal control framework to coordinate CAVs and HDVs at any traffic scenario. The idea is to directly control the CAVs to force the trailing HDVs to form platoons. Thus, we indirectly control the HDVs by coordinating the platoon of HDVs led by CAVs.

==> 4broader_impacts.tex <==

\textbf{Impact on Society:}
Emerging mobility systems, e.g., CAVs, shared mobility, provide the most intriguing opportunity for enabling users to better monitor transportation network conditions and make better decisions for improving \textbf{safety} and \textbf{transportation efficiency} \cite{zhao2019enhanced}. 
The  data and shared information through vehicle-to-vehicle and vehicle-to-infrastructure communication are associated with significant technical challenges and gives rise to a new level of complexity in modeling and control \cite{Ferrara2018}. 
It is expected that CAVs will gradually \textbf{penetrate} the market and interact with HDVs in way to improve safety and transportation efficiency \cite{Malikopoulos2018d, Zhao2018CTA, cassandras2019b} over the next several years. However, different levels of vehicle automation  in the transportation network can significantly alter  transportation efficiency  ranging for 45\% improvement to 60\% deterioration \cite{wadud2016}.  
The theoretical framework developed in the proposed research will aim at facilitating optimal solutions with performance guarantees to allow safe co-existence of CAVs with HDVs while improving transportation efficiency.

\textbf{Impact on Education and Outreach:} The proposed research is an excellent catalyst for motivating interest in  science, technology, engineering, and mathematics (STEM) disciplines, for which there is a nationally recognized need for improvement. 
The PI has invested in the past, and will continue to invest, time and resources in broadening the participation of students, especially under-represented population in STEM fields in general.  He has been also a coach on First Tech Challenge (FTC) since 2019 mentoring a group of middle and high-school students. The PI regularly mentors high-school students through the UD K12 program (this program brings on campus high-school students for summer internships). 
The UD's scaled smart city testbed has attracted the attention of local high-school students who are currently involved in research activities in the PI's lab. This project will engage several high-school students through the UD K12 program and host undergraduate students from universities worldwide. Luke Bhan, currently a junior at Vanderbilt University, joined the PI's lab in the summer of 2017 through the UD K12 program to conduct research on CAVs resulting in being the second author in a paper that was presented in the 15th IFAC Symposium on Control in Transportation Systems \cite{Malikopoulos2018b}. Lucas Ramsey (UD K12 program in 2018) is now a sophomore in computer science at the University of Michigan. Christophoros Kontomaris (UD K12 program in 2018 and 2019) is now a freshman in mechanical engineering at Georgia Institute of Technology. The outreach events will benefit from the PI's previous experiences and training. The PI has received training in inclusive teaching through a series of modules from the diversity and inclusion committee of UD's College of Engineering. He is committed to using summer scholars on this project along with other undergraduate students already included in the budget. 

\textbf{Proposed efforts:} In this project the PI plans to (i) train graduate students by exposing them to a balanced mix of theory and practice, (ii) integrate the proposed research into existing courses, (iii) involve undergraduate students, especially under-represented population, in research, (iv) create interactive educational demos, and (v) reach out to high-school students. In particular, for (ii), the PI teaches graduate and advanced undergraduate level courses \emph{MEEG 698 Stochastic Optimal Control} and  \emph{MEEG 890 Nonlinear Programming}. Results from this project will be included in examples to demonstrate the foundational theory and also be included in the list of possible term projects. For (iii), the proposed work provides an excellent opportunity for undergraduates to get involved in the
research through participating in the testing and validation effort on UD's scaled smart city testbeds where much of our testing will be conducted. The PI will  support undergraduate researchers through each calendar year, including the summer. These students will primarily participate in the testing and validation effort, using the experimental testbeds described in the Facilities, Equipment, \& Other Resources section. In addition to direct mentoring by the PI, the undergraduates will work closely with the PhD students involved in the project and attend the group meetings of the PI to get a more complete view of the research programs. Finally, for (iv) and (v) the PI will also continue his efforts with demonstrations at UD's K12 program. In all these activities, the physical testbeds will play a key role, providing a visual demonstration of the ideas behind the algorithms and giving the students the opportunity to work on algorithm deployment and testing, to learn about topics including optimization, optimal control, machine learning, programming, and to conduct research.


==> 5prior_nsf_ri.tex <==

\textbf{Malikopoulos:} CNS-2149520 (7/22--6/25, \$1,179M, Co-PIs: C. Cassandras and C. Wu).
\emph{Intellectual Merit:} This work establishes new approaches in optimally controlling cyber-physical systems (CPS) by merging learning and control approaches. It includes the development of new methods to enhance accessibility, safety, and equity in transportation and travelers’ acceptance, as well as to bridge the gap between optimal trajectory planning and safety-critical control in CPS. 
\emph{Broader Impact:} The project will consolidate emerging mobility systems and modes such as CAVs and ride-share services with real-world data and processed information, that will yield broad economic, environmental, and societal effects. This research will advance the state of the art combining optimal and safe control methods in conjunction with new mechanism design techniques and learning methods.

==> 6data_management_ri.tex <==
\\

Metadata for project data will be assigned in accordance with established
metadata standards and best practices. The Dublin Core Metadata Initiative
specification and standards (\url{http://dublincore.org/}) will be
investigated and applied whenever possible.

\noindent \textbf{Computational results:} Computations and simulations
conducted in this project will generate large sets of data. We plan to make
the source code of our algorithms available and the input data when the
latter is possible. Output datasets that are computationally demanding to
reproduce will be archived and made publicly available.

\noindent \textbf{Educational materials:} Research in this project is related to several UD 
courses, most notably \emph{MEEG 698 Stochastic Optimal Control} and \emph{MEEG 890 Nonlinear Programming}
regularly taught by Malikopoulos. The expected data to be generated and
retained during the course of this project includes textual materials which
will be published in theses, books, book chapters, journals, and/or
conference publications, both in print and electronic formats (PDF). Sample
experimental datasets will also be published in CSV format to enable easy
access to researchers working in various computing environments (Excel,
MATLAB, Python, etc.).

\subsection*{Policies for Access and Sharing and Provisions for Appropriate
Protection/Privacy}

The data generated for this project will be retained for a minimum period of
three years after the conclusion of the award. All software is permanently
archived on \textsf{GitHub}.

\subsection*{Policies and Provisions for Re-use, Re-distribution of Data}

Redistribution and reuse of software will require a default license. We will use Creative Commons licensing (http://creativecommons.org/) as a system because it is organized and rational. 
Use of products generated from this grant must clearly recognize the developer and NSF in any subsequent publications or presentations. 
Similarly, remixing and adapting materials is permissible, but requires recognition of original authors.
Small datasets and any necessary software toolboxes will be hosted or linked
from the PIs web sites. The PIs will share results, including software,
testbeds, and other artifacts.

\noindent \textbf{Creation of publicly available software:} Open source
codes produced by the team, will be made publicly available via the web, for
example at \textsf{GitHub} for source codes.

\textbf{Web site:} Data and code produced by the PI will be made available at 
\textsf{GitHub} and linked through the PI's research group web site (%
\url{http://sites.udel.edu/ids-lab/}).

\textbf{Plans for Archiving and Preservation of Access:} The University of Delaware (UD) has a number of services and facilities for data management. In
particular, UD Libraries provide guidelines that cover the general
principles for managing data from research projects, in compliance with
federal mandates and expectations of ethical research conduct. For curation and archiving,
UD maintains a Digital Common, in which documents and
publications authored or co-authored by UD faculty, students, and staff are
archived. 

\subsection*{Policies for Dissemination and Sharing of Research Results}

The researchers are not required to make all these data available publicly
but will do so upon request from other interested parties in accordance with
the normal course of research.

\textbf{Publications:} Research results will be published in appropriate
journals; results will be disseminated to peer-researchers via presentations
and email. In research articles, a particular effort will be taken to make
the results as easily reproducible as possible. Unless prohibited by
proprietary rights, software and data produced in this research will be
permanently archived via \textsf{GitHub}, enabling the reader/user to
reproduce the results.



==> 7facilities_ri.tex <==
\\
\setcounter{figure}{0}
\subsection*{Computing Facilities}
The project will  utilize the computing infrastructure at the University of Delaware (UD). UD has extensive computing facilities that are devoted to the research needs of the UD faculty and students. A recent computing facility is Caviness. Caviness was deployed in July 2018 and is a distributed-memory Linux cluster. It consists of 126 compute nodes (4536 cores, 24.6 TB memory). The nodes are built of Intel ``Broadwell'' 18-core processors in a dual-socket configuration for 36-cores per node. An OmniPath network fabric supports high-speed communication and the Lustre filesystem (approx. 200 TiB of usable space). Gigabit and 10-Gigabit Ethernet networks provide access to additional filesystems and the campus network.

\subsection*{Driver Simulation Testbed}

The proposed work will leverage the facilities and equipment of the lead PI's Information and Decision Science (IDS) Laboratory. IDS houses state-of-the-art, high-end PCs supporting standard software for system analysis and optimization, as well as more specialized simulation tools for transportation, communication networks, and multi-agent systems. 
IDS facilities include  a \textbf{driver simulation testbed} (Figure \ref{sim}) with six driver simulators that can accommodate human-driven vehicles all linked together in a transportation environment and projected on a 75-inch monitor. This environment can include connected and automated vehicles (CAVs) and represent any city, or region in the world. The driver simulation testbed can help us study the coordination between different penetrations rates of CAVs and their interaction with human-driven vehicles as well as implications regarding energy usage, emissions, safety, and travel time.

\begin{figure}[h]
	\centering
	\includegraphics
	[width=0.9\textwidth]
	{driver.png}
	\caption{\small The simulation testbed with six driver simulators.
	}
	\label{sim}
\end{figure}

\subsection*{IDS Lab's Scaled Smart City (IDS$^3$C)}

IDS facilities include the  \textbf{IDS Lab's Scaled Smart City (IDS$^3$C) (1:25)} (Figure \ref{udssc}). IDS$^3$C occupies a 20 by 20 feet area. It includes 50 robotic vehicles and can replicate real-world traffic scenarios in a small and controlled environment. This testbed can help us prove concepts beyond the simulation level and understand the implications of errors/delays in the vehicle-to-vehicle and vehicle-to-infrastructure communication as well as their impact on energy usage. IDS$^3$C can  help us implement control algorithms for coordinating CAVs in different traffic scenarios, such as intersections\footnote{https://sites.google.com/view/ud-ids-lab} (Figure \ref{cav}), merging roadways, speed reduction zones, and roundabouts. 
IDS$^3$C has 6 \textbf{driver emulation stations\footnote{https://www.youtube.com/watch?v=f5ZRQLLQirE}} (Figure \ref{driver}) interfaced directly with the robotic cars which allow us to explore human driving behavior using robotic cars.


\begin{figure}[t]
	\centering
	\includegraphics
	[width=0.7\textwidth]
	{udssc.jpg}
	\caption{\small
		A view of the University of Delaware's scaled smart city.
	}
	\label{udssc}
\end{figure}


\begin{figure}[h]
	\centering
	\includegraphics
	[width=0.5\textwidth]
{driver2.pdf}
\caption{\small A driver emulation station interfaced directly with the robotics vehicles and allow to explore human driving behavior in the scaled city.
}
\label{driver}
\end{figure}


\begin{figure}[h]
	\centering
	\includegraphics
	[width=0.9\textwidth]
	{CAV.pdf}
	\caption{\small Coordination of robotic connected and automated vehicles at an urban intersection having a drone acting as the coordinator. 
	}
	\label{cav}
\end{figure}

The robotic CAVs of IDS$^3$C  (Figure \ref{fig:CAV}) have been designed using off the shelf electrical components and $3$D printed parts created at UD. The primary microcontroller on the CAV is a Raspberry Pi $3$B running Ubuntu Mate and ROS Kinetic. An Arduino Nano is used as a slave processor for the Pi to do low-level motor control and ad-hoc analog to digital conversion for the state of charge (SOC) measurements. The CAV's rear-wheel drivetrain is powered by a Pololu $75.8$:$1$, $6$ V micro metal gearmotor; the motor is controlled using a motor controller, and encoder for feedback, through the Arduino. Power from the gear-motor is transferred to the rear axle with two $3$D printed gears with a $1$:$1$ ratio, and two rubberized wheels with radius $r=1.6$ cm are mounted directly to the rear axle. The motor controller receives power through a $5$ V regulator, and a pulse-width modulated command from the Arduino is used to control the motor's speed. Steering is achieved by a custom $3$D printed Ackermann-style steering mechanism actuated by a Miuzei micro servo motor, which again is controlled directly by the Arduino. The CAVs are also equipped with a Pi Camera, ultrasonic sensors, and a SOC measurement circuit to collect experimental data and reduce the overall reliance on VICON. A power regulator manages the voltage requirement of the Pi and Arduino by supplying a regulated $5$ V DC from two $3000$ mAh $3.7$ V Li-ion batteries configured in series. With this hardware configuration, the CAV is able to run and collect experimental data at $20$ Hz for up to $2$ hours.


IDS$^3$C has a multi-level control architecture with high level commands originating from a centralized PC (Processor: Intel Core i7-6950X CPU @ 3.00 GHz x 20, Memory: 125.8 GiB) then enforced by a low-level controller on-board each robotic vehicle. Asynchronous communication is enabled by WiFi connectivity using the Node.js non-blocking I/O protocol. Electron uses a socket server with a socketIO library natively supporting multi-threading for multi-vehicle communication. A web browser combines JavaScript, HTML for a user friendly interface into the \textbf{ROS architecture.} 

Coordination of the CAVs within the IDS$^3$C is achieved using a multi-level control framework spanning a central \textit{mainframe} computer  and the individual CAVs (Raspberry Pi 3B). The mainframe runs an Ubuntu 16.04.5 LTS Linux distribution and ROS Kinetic. High-level routing is achieved by a multithreaded C++ program running on the mainframe computer. The mainframe is initialized with the path information and speed profiles for each CAV. At the start of the experiment, each CAV sets its temporal baseline from which it measures all later times; this avoids the problem of synchronizing CAV clocks, as all information is calculated relative to the experiment start time. During the experiment, the mainframe passes a message to each CAV containing its current position and two seconds of trajectory data using the UDP/IP protocol at $50$ Hz. The CAV receives trajectory information from the mainframe and uses a modified Stanley \cite{Thrun2007Stanley:Challenge} controller to handle lane tracking, while a feedforward-feedback \cite{Spong2004RobotEdition} PID controller tracks the desired speed profile.

\begin{figure}
	\begin{minipage}{\linewidth}
		\includegraphics[height=2.5in]{figures/CAV-noshell.png}\hfill
		\includegraphics[height=2.5in]{figures/CAV-v3.png}%
	\end{minipage}
	\caption{A picture of the connected and automated vehicle's electronics (left) and outer shell with VICON markers, ultrasonic sensors, and camera visible (right).}
	\label{fig:CAV}
\end{figure}


Medium and low-level control is accomplished onboard each CAV in a purely distributed manner. Using information from the mainframe, each %vehicle's Raspberry Pi
CAV updates at $50$ Hz to calculate a lateral, heading, and distance error. The lateral and heading errors are then passed to the Stanley controller to calculate an output steering angle. Meanwhile, the position error and desired speed are used in a feedforward-feedback controller to calculate the desired motor speed. The desired speed and steering angle are then passed to the Arduino Nano, which runs a low-level PID controller to precisely control the gear-motor and steering servo.

IDS$^3$C can also be operated in a \textbf{virtual simulation environment} that facilitates (1) working remotely and (2) using it as a practical debugging tool for implementing new control algorithms. The simulation uses Microsoft AirSim and the Unity game engine to handle physics and low-level control of the robotic vehicles, which are commanded by a custom lane tracking script used by each virtual robotic vehicle. The virtual vehicle receives high-level routing information through a ROS nodelet, which includes the desired lane and speed information for the vehicle. Each virtual vehicle is also equipped with position and velocity sensors as well as a virtual camera. The data from these sensors are published to a ROS topic by each vehicle, where they can be accessed by any external ROS application. This allows us to hook the virtual simulation environment directly into our existing control code, while also enabling its use for computer vision applications.

The testbeds of the IDS Lab have attracted the attention of local high school students who are currently involved in research activities\footnote{https://outreachidssc.wixsite.com/outreach}. These physical testbeds will play a key role, providing a visual demonstration of the ideas behind the algorithms and giving exceptional high school students the opportunity to conduct research.

Additional information on IDS Lab may be found at \textbf{https://sites.udel.edu/ids-lab/}

\subsection*{Mcity at the University of Michigan}

To evaluate our proposed work with full-scale field testing, we will use the University of Michigan's Mcity (Fig. \ref{fig:mcity2})  and Mcity's Lincoln MKZ CAV. The PI has used Mcity in several projects in the past in collaboration with the director of Mcity, Professor Henry Liu \textbf{(see collaboration letter).}

Mcity is a full-scale urban environment designed for testing the performance and safety of CAVs under controlled and realistic road conditions. It is a 32-acre outdoor laboratory for advanced mobility systems that  includes:
\begin{enumerate}
	\item Urban and suburb streets, including various lane configurations and sidewalks, pedestrian crossings, bike lanes, ADA ramps, street lights, parallel and diagonal parking, and a bus turnoff/stop.
	\item Instrumentation throughout, including a control network to collect data about traffic activity using wireless, fiber optics, Erthenet, and a highly accurate real-time kinematic positioning systems.
\end{enumerate}

\begin{figure}[h]
	\centering
	\includegraphics
	[width=0.4\textwidth]
	{mcity.png}
	\caption{University of Michigan's Mcity}
	\label{fig:mcity2}
\end{figure}




The project will leverage also several other resources and expertise of the Sociotechnical Systems Center (SSC) at UD. SSC is a collaborative and interdisciplinary community at UD with shared research interests and goals in addressing complex problems. The mission of SSC is to develop rigorous, system-based approaches aimed at addressing current challenges founded at the intersection of technological, social, and institutional dimensions.

Additional information on SSC may be found at \textbf{https://sites.udel.edu/engr-ssc/}


==> 8BPC.tex <==
\\
\setcounter{figure}{0}
\begin{wrapfigure}{r}{0.5\textwidth}
	\vspace{-2ex}
	\centering
	\includegraphics
	[width=0.5\textwidth]
	{andreas_first.jpg}
	\caption{\small
		 Meeting of Malikopoulos' FTC team at his lab in UD.
	}
	\label{fig:first}
	\vspace{-2ex}
\end{wrapfigure}

There is a large appeal and interest in cyber-physical systems (CPS) research among the younger generation. Thus,  we believe that the proposed research is an excellent catalyst for motivating interest in science, technology, engineering, and mathematics (STEM) disciplines, for which there is a nationally recognized need for improvement. The natural appeal of CPS can be leveraged to help bring important scientific and engineering principles into the public eye and facilitate education. 
The PI has invested in the past, and will continue to invest, time and resources in broadening the participation of students, especially students from historically underrepresented groups, in the proposed STEM fields in general. The PI regularly mentors high-school students through the UD K12 program (this program brings high school students to campus for summer internships) and hosts undergraduate students from universities worldwide. He has also been a coach on First Tech Challenge (FTC) since 2019, mentoring a group of middle and high school students (Fig. \ref{fig:first}). 

This project will engage several high school students through the UD K12 program and host undergraduate students from universities worldwide. Several high school students who participated in UD's K12 program under PI's advising are currently in college. Luke Bhan (UD K12 program in 2017) is currently a junior at Vanderbilt University. Lucas Ramsey (UD K12 program in 2018) is now a sophomore in computer science at the University of Michigan. Christophoros Kontomaris (UD K12 program in 2018 and 2019) is now a freshman in mechanical engineering at Georgia Institute of Technology. The outreach\footnote{https://outreachidssc.wixsite.com/outreach} events will benefit from the PI's previous experiences and training. The PI has received training in inclusive teaching through a series of modules from the diversity and inclusion committee of UD's College of Engineering. He is committed to using summer scholars on this project along with other undergraduate students already included in the budget. 


The broadening participation efforts will benefit from the PI's previous experiences and training.  In this project, we plan to (1) focus on training particularly students from underrepresented groups and female undergraduate and high-school students over the summer by exposing them to applied projects and (2) integrate the proposed research into tutorial courses that can be offered in summer camps. In particular,  the PI teaches the undergraduate course \emph{MEEG 311 Control Systems}. Results from this project will be used to create a new course appropriate for high-school students in UD's K12 summer program. The proposed work also provides an excellent opportunity for undergraduate and high-school students to get involved through participating in the testing and validation efforts on the driver simulation and the scaled smart city testbeds where much of our testing will be conducted. The PIs will each support undergraduate researchers through each calendar year, including the summer. These students will primarily participate in the testing and validation efforts, using the experimental testbeds described in the Facilities, Equipment, \& Other Resources section. In addition to direct mentoring by the PIs, the undergraduates will work closely with the PhD students involved in the project and attend the group meetings of the PIs to get a more complete view of the research programs. In all these activities, the physical testbeds will play a key role, providing a visual demonstration of the ideas behind the algorithms and giving the exceptional high-school students the opportunity to work on algorithm deployment and testing, to learn about topics including optimization, dynamics, and programming, and to participate in the research.


\textbf{Metrics of Success.} The assessment of all the broadening participation efforts will be done via the UD's K12 program. These programs have already established mechanisms for hosting students and monitoring their overall performance in STEM-related activities. The metrics to measure the progress and success of the proposed plan will be both summative, in that it will assess the extent to which the final outcomes for each effort address the outcomes stated in the goals, as well as formative, in that it will assess the procedures and methods that will lead to these outcomes.  
The validation of the proposed framework in the scaled city will  help us create educational materials that can be used for high school and undergraduate students. The desired traffic scenarios of the robotic cars within the scaled city will be chosen by the students.  These experiments will help the high school and undergraduate students become familiar with the technological implications of CPS. 




